The Shortest Path to Happiness: Recommending Beautiful, Quiet, and Happy Routes in the City

When providing directions to a place, web and mobile mapping services are all able to suggest the shortest route. The goal of this work is to automatically suggest routes that are not only short but also emotionally pleasant. To quantify the extent to which urban locations are pleasant, we use data from a crowd-sourcing platform that shows two street scenes in London (out of hundreds), and a user votes on which one looks more beautiful, quiet, and happy. We consider votes from more than 3.3K individuals and translate them into quantitative measures of location perceptions. We arrange those locations into a graph upon which we learn pleasant routes. Based on a quantitative validation, we find that, compared to the shortest routes, the recommended ones add just a few extra walking minutes and are indeed perceived to be more beautiful, quiet, and happy. To test the generality of our approach, we consider Flickr metadata of more than 3.7M pictures in London and 1.3M in Boston, compute proxies for the crowdsourced beauty dimension (the one for which we have collected the most votes), and evaluate those proxies with 30 participants in London and 54 in Boston. These participants have not only rated our recommendations but have also carefully motivated their choices, providing insights for future work.

==> 07_related.tex <==
The problem of recommending events has been initially tackled on the Web. In this context, researchers have mainly worked on detecting and tracking events~\cite{Ihler06adpative,Kleinberg02bursty}.  They initially  considered how textual content evolves over  time and left out network effects. Zhu and Sasha then started to model social interactions and topic evolutions by treating these two elements separately~\cite{Zhou06topic}. More recently, Lin \emph{et al.} built a model that considers these two elements simultaneously and showed that it worked upon two very different types of data - Twitter and DBLP~\cite{Lin10pet}. After detecting events, one can  then recommend them. That is what Daly and Geyer \emph{et al.} did: they built a system that recommends events in an internal event management service and proposed a new way of recommending events to new users~\cite{Daly11effective}.  Before that, Minkov \emph{et al.} had run large user studies in which they evaluated the effectiveness of different strategies for recommending academic talks~\cite{Minkov10collaborative}. They found that, in a situation of limited data sparsity, collaborative filtering approaches work better than content-based ones. The recommendation process generally relies on user ratings but has also been enriched by social networks at times. A case in point  is Golbeck \emph{et al.} who built a recommender system  that integrates social networks to offer well-informed movie recommendations~\cite{Golbeck09trust}.	

Hence past work on recommending events has mostly gone into Web platforms, while mobile ones have  been investigated only recently.  Takeuchi and Sugimoto proposed a system that recommends shops based on past visited locations, and found item-based collaborative filtering to work reasonably well~\cite{yuichiro06city}.  Ricci and Nguyen proposed a system that recommend nearby restaurants using a critique-based model~\cite{Ricci07acquiring}. More recently, for major mobile social networking services, Scellato \emph{et al.} studied their geographic properties at scale and suggested that these properties could well inform venue recommendation in large cities~\cite{scellato11socio}. Upon mobile phone data in the metropolitan area of Boston, Quercia \emph{et al.} studied strategies for recommending large-scale events (e.g., concerts, baseball matches) and showed how different types of events require different recommendation strategies~\cite{quercia10recommending}.

Shifting attention from recommending events to recommending people, one sees that most of the work has again gone into  Web platforms. Within an enterprise social network, Guy \emph{et al.} proposed ways to recommend people a user is not likely to know but might be interested in~\cite{Guy11doyou}. Few months ago, Facebook launched a new feature called ``suggested guests''~\cite{darwell12}: this returns a list of people (three at the time) a user might want to consider inviting to their event, and the list is compiled based on relevance to the event and to the people who are attending. Since work on recommending people for events has just started on the Web, it  comes as no surprise that little work about it has gone into mobile social networking platforms.
